Smoothness Similarity Regularization for Few-Shot GAN Adaptation

The task of few-shot GAN adaptation aims to adapt a pre-trained GAN model to a small dataset with very few training images. While existing methods perform well when the dataset for pre-training is structurally similar to the target dataset, the approaches suffer from training instabilities or memorization issues when the objects in the two domains have a very different structure. To mitigate this limitation, we propose a new smoothness similarity regularization that transfers the inherently learned smoothness of the pre-trained GAN to the few-shot target domain even if the two domains are very different. We evaluate our approach by adapting an unconditional and a class-conditional GAN to diverse few-shot target domains. Our proposed method significantly outperforms prior few-shot GAN adaptation methods in the challenging case of structurally dissimilar source-target domains, while performing on par with the state of the art for similar source-target domains.

==> figures/biggan_old.tex <==
\begin{figure*}[t]
\begin{centering}
\setlength{\tabcolsep}{0.01in}
\renewcommand{\arraystretch}{1}
\par\end{centering}
\begin{centering}
%\hfill{}%

%%%%%%%%%% first 
\begin{tabular}{
@{\hskip -0.02in} c @{\hskip 0.10in} c @{\hskip 0.10in} c@{\hskip 0.00in} }

Real samples -- 10-Shot \color{purple} Flowers \color{black} & Real samples -- 10-Shot \color{brown} Pokemons \color{black} & Real samples -- 10-Shot \color{teal} Moongate \color{black} \color{black}
\tabularnewline[0pt]

\includegraphics[draft=\draft,width=0.320\linewidth]{figures/qualitative_results/imagenet-flowers/ref/ref_flowers.jpg} &
\includegraphics[draft=\draft,width=0.320\linewidth]{figures/qualitative_results/imagenet-pokemon/ref/ref_pokemons.jpg} &
\includegraphics[draft=\draft,width=0.320\linewidth]{figures/qualitative_results/imagenet-moongate/ref/ref_moongate.jpg}
\tabularnewline[1pt]
\end{tabular}


%%%%%%%%%% second
\begin{tabular}{ @{\hskip -0.13in} c @{\hskip 0.05in}
c @{\hskip 0.01in} c @{\hskip 0.01in} c @{\hskip 0.01in} c @{\hskip 0.01in} c @{\hskip 0.01in} c @{\hskip 0.01in} c @{\hskip 0.01in} c @{\hskip 0.01in} c@{\hskip 0.01in} c @{\hskip 0.01in} c @{\hskip 0.01in} c @{\hskip 0.01in} c @{\hskip 0.01in} c @{\hskip 0.01in} }

& \multicolumn{14}{c}{10-Shot adaptation results of our method on class-conditional BigGAN \cite{Brock2019}, pre-trained on ImageNet}
\tabularnewline[0pt]

~~\rotatebox{90}{{\hspace{0.3em} \small Source \hspace{0.0em} }} &
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_570.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_580.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_586.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_591.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_601.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_611.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_622.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_633.jpg}} & \frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_645.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_654.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_665.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_673.jpg}} & \frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_682.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-art-paiting/source/z1_693.jpg}} \tabularnewline[-0pt]

~~\rotatebox{90}{{\hspace{0.2em} \color{purple} \small Flowers \color{black} \hspace{-1.0em} }} &
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_571.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_580.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_586.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_591.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_601.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_616.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_630.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_645.jpg}} & \frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_654.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_664.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_670.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_675.jpg}} & \frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_681.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-flowers/ours/z3_695.jpg}} 
\tabularnewline[-3pt]

~~\rotatebox{90}{{\hspace{-0.5em} \color{brown} \small Pokemons \color{black} \hspace{-1.0em} }} &
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_570.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_580.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_586.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_591.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_601.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_606.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_616.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_630.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_894.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_928.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_940.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_955.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_964.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-pokemon/ours/z2_979.jpg}}
\tabularnewline[-3pt]

~~\rotatebox{90}{{\hspace{-0.15em} \color{teal} \small Moong. \color{black} \hspace{-1.0em} }} &
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_570.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_580.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_586.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_601.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_616.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_630.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_645.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_654.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_665.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_670.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_675.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_681.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_682.jpg}} & 
\frame{\includegraphics[draft=\draft,width=0.0684\linewidth, height=0.0684\linewidth]{figures/qualitative_results/imagenet-moongate/ours/z3_695.jpg}} 
\tabularnewline[-3pt]
\end{tabular}




\par\end{centering}
\vspace{5pt}
\caption{10-shot adaptation results on class-conditional BigGAN \cite{Brock2019}, pre-trained on ImageNet. Despite the extremely low data regime and a significant structural dissimilarity between ImageNet and target domains, our method achieves both high quality and diversity, transferring smooth and realistic image transitions from the source domain, e.g., objects smoothly changing their locations, size, and shape.}
\label{fig:qualitative_biggan}

\end{figure*}

==> figures/plots_metrics2.tex <==
\begin{figure*}[t]
\begin{centering}
\setlength{\tabcolsep}{0.53in}
\renewcommand{\arraystretch}{1}
\par\end{centering}
\begin{centering}
%\hfill{}%
%\vspace{-0.5ex}
\begin{tabular}{@{\hskip -0.05in}c@{\hskip 0.00in}c@{\hskip 0.00in}c@{\hskip 0.00in}c@{\hskip 0.00in}}


\includegraphics[width=0.47\linewidth, height=0.35\linewidth]{figures/plots_metrics/plot_fid_fid1.jpg} ~~~
\includegraphics[width=0.47\linewidth, height=0.35\linewidth]{figures/plots_metrics/plot_fid_lpips1.jpg} 

\end{tabular}

\par\end{centering}
\caption{The FID and LPIPS curves of different methods for the few-shot adaptation between close domains \textit{Face$\rightarrow$Sunglasses}.
}
\label{fig:plots_metrics2}
%\vspace{-1.5ex}
\end{figure*}

==> figures/qual_comparison_close3.tex <==
\begin{figure}[t]
\begin{centering}
\setlength{\tabcolsep}{0.01in}
\renewcommand{\arraystretch}{1}
\par\end{centering}
\begin{centering}
%\hfill{}%

%%%%%%%%%% first 
\begin{tabular}{@{\hskip -0.13in}c@{\hskip 0.10in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c:c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c}

~~\rotatebox{90}{{\hspace{0.0em} Real \hspace{0.0em} }} &

\multicolumn{7}{@{\hskip -0.04in}c:}{
\frame{\includegraphics[width=0.0930\linewidth, height=0.0930\linewidth]{figures/qualitative_results/church-vangogh/ref/00117.jpg}} \hspace{-1.0ex}
\frame{\includegraphics[width=0.0930\linewidth, height=0.0930\linewidth]{figures/qualitative_results/church-vangogh/ref/00195.jpg}} \hspace{-1.0ex}
\frame{\includegraphics[width=0.0930\linewidth, height=0.0930\linewidth]{figures/qualitative_results/church-vangogh/ref/00220.jpg}} \hspace{-1.0ex}
\frame{\includegraphics[width=0.0930\linewidth, height=0.0930\linewidth]{figures/qualitative_results/church-vangogh/ref/00242.jpg}} \hspace{-1.0ex}
\frame{\includegraphics[width=0.0930\linewidth, height=0.0930\linewidth]{figures/qualitative_results/church-vangogh/ref/00262.jpg}} \hspace{-1.0ex}
\frame{\includegraphics[width=0.0930\linewidth, height=0.0930\linewidth]{figures/qualitative_results/church-vangogh/ref/00519.jpg}} \hspace{-1.0ex}
\frame{\includegraphics[width=0.0930\linewidth, height=0.0930\linewidth]{figures/qualitative_results/church-vangogh/ref/00536.jpg}} \hspace{-1.0ex}
\frame{\includegraphics[width=0.0930\linewidth, height=0.0930\linewidth]{figures/qualitative_results/church-vangogh/ref/00654.jpg}} \hspace{-1.0ex}
\frame{\includegraphics[width=0.0930\linewidth, height=0.0930\linewidth]{figures/qualitative_results/church-vangogh/ref/00697.jpg}} \hspace{-1.0ex}
\frame{\includegraphics[width=0.0930\linewidth, height=0.0930\linewidth]{figures/qualitative_results/church-vangogh/ref/00247.jpg}}  
} 

\tabularnewline[2pt]

~~\rotatebox{90}{{\hspace{0.0em} Source \hspace{-3.0em} }} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-hh/source/p_1_000000.jpg}} & 
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-hh/source/p_3_000000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-hh/source/p_5_000000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-hh/source/p_6_000000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-hh/source/p_12_000000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-hh/source/p_16_000000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-hh/source/p_17_000000.jpg}}
\tabularnewline[-3pt]


~~\rotatebox{90}{{\hspace{0.4em} CDC \hspace{-3.0em} }} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/cdc/p_1_001500.jpg}} & 
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/cdc/p_3_001500.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/cdc/p_5_001500.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/cdc/p_6_001500.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/cdc/p_12_001500.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/cdc/p_16_001500.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/cdc/p_17_001500.jpg}} 
\tabularnewline[-3pt]


~~\rotatebox{90}{{\hspace{0.3em} RSSA \hspace{-3.0em} }} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/rssa/p_1_002500.jpg}} & 
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/rssa/p_3_002500.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/rssa/p_5_002500.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/rssa/p_6_002500.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/rssa/p_12_002500.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/rssa/p_16_002500.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/rssa/p_17_002500.jpg}} 
\tabularnewline[-3pt]


~~\rotatebox{90}{{\hspace{0.1em} AdAM \hspace{-3.0em} }} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/adam/p_1_001000.jpg}} & 
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/adam/p_3_001000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/adam/p_5_001000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/adam/p_6_001000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/adam/p_12_001000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/adam/p_16_001000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/adam/p_17_001000.jpg}} 
\tabularnewline[-3pt]


~~\rotatebox{90}{{\hspace{0.4em} Ours \hspace{-3.0em} }} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/ours/p_1_001000.jpg}} & 
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/ours/p_3_001000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/ours/p_5_001000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/ours/p_6_001000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/ours/p_12_001000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/ours/p_16_001000.jpg}} &
\frame{\includegraphics[width=0.134\linewidth, height=0.134\linewidth]{figures/qualitative_results/church-vangogh/ours/p_17_001000.jpg}} 
\tabularnewline[-3pt]


\end{tabular}
\par\end{centering}
\vspace{5pt}
\caption{Additional visual comparison to most recent prior methods on related domains.}
\label{fig:qualitative_comparison_close3}

\end{figure}

==> figures/qual_comparison_distant2.tex <==
\begin{figure*}[t]
\begin{centering}
\setlength{\tabcolsep}{0.53in}
\renewcommand{\arraystretch}{1}
\par\end{centering}
\begin{centering}
%\hfill{}%

%%%%%%%%%% first 
\begin{tabular}{@{\hskip -0.02in}c@{\hskip 0.04in}:c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{\hskip 0.01in}c}

  \multirow{-1}{*}{\begin{tabular}{c@{\hskip 0.01in}c@{\hskip 0.03in}} 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ref/2.jpg}} &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ref/5.jpg}} \tabularnewline[-3pt]	
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ref/25.jpg}} &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ref/30.jpg}} \tabularnewline[-3pt]	
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ref/32.jpg}} &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ref/40.jpg}} \tabularnewline[-3pt]	
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ref/48.jpg}} &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ref/70.jpg}} \tabularnewline[-3pt]	
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ref/97.jpg}} &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ref/136.jpg}} \tabularnewline[+1pt]	
  \multicolumn{2}{@{\hskip -0.02in}c@{\hskip 0.03in}}{\small 10-shot} \tabularnewline[-2pt] 
  \multicolumn{2}{@{\hskip -0.02in}c@{\hskip 0.03in}}{\small Anime-Faces} \tabularnewline[-3pt]
  \end{tabular}} &
  
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/TGAN/p_1_001000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/TGAN/p_3_001000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/TGAN/p_4_001000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/TGAN/p_5_001000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/TGAN/p_7_001000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/TGAN/p_8_001000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/TGAN/p_10_001000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/TGAN/p_18_001000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/TGAN/p_21_001000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/TGAN/p_25_001000.png}} & ~~\rotatebox{270}{{\hspace{-3.6em} TGAN \hspace{-3.0em} } }
  \tabularnewline[-3pt]
  &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/freezeD/p_1_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/freezeD/p_3_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/freezeD/p_4_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/freezeD/p_5_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/freezeD/p_7_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/freezeD/p_8_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/freezeD/p_10_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/freezeD/p_18_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/freezeD/p_21_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/freezeD/p_25_001500.png}} & ~~\rotatebox{270}{{\hspace{-3.7em} FreezeD \hspace{-3.0em} } }
  \tabularnewline[-3pt]
  &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/cdc/p_1_003000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/cdc/p_3_003000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/cdc/p_4_003000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/cdc/p_5_003000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/cdc/p_7_003000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/cdc/p_8_003000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/cdc/p_10_003000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/cdc/p_18_003000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/cdc/p_21_003000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/cdc/p_25_003000.png}} & ~~\rotatebox{270}{{\hspace{-3.0em} CDC \hspace{-3.0em} } }
  \tabularnewline[-3pt]
  &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/rssa/p_1_004000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/rssa/p_3_004000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/rssa/p_4_004000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/rssa/p_5_004000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/rssa/p_7_004000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/rssa/p_8_004000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/rssa/p_10_004000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/rssa/p_18_004000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/rssa/p_21_004000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/rssa/p_25_004000.png}} & ~~\rotatebox{270}{{\hspace{-3.2em} RSSA \hspace{-3.0em} } }
  \tabularnewline[-3pt]
  &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/adam/p_1_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/adam/p_3_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/adam/p_4_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/adam/p_5_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/adam/p_7_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/adam/p_8_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/adam/p_10_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/adam/p_18_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/adam/p_21_001500.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/adam/p_25_001500.png}} & ~~\rotatebox{270}{{\hspace{-3.4em} AdAM \hspace{-3.0em} } }
  \tabularnewline[-3pt]
  &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ours/p_2_026000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ours/p_3_026000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ours/p_4_026000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ours/p_5_026000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ours/p_7_026000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ours/p_8_026000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ours/p_10_026000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ours/p_18_026000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ours/p_21_026000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/ours/p_25_026000.png}} & ~~\rotatebox{270}{{\hspace{-3.1em} \textbf{Ours} \hspace{-3.0em} } }
  \tabularnewline[-3pt]
  &
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/source/p_2_000000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/source/p_3_000000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/source/p_4_000000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/source/p_5_000000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/source/p_7_000000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/source/p_8_000000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/source/p_10_000000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/source/p_18_000000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/source/p_21_000000.png}} & 
  \frame{\includegraphics[width=0.075\linewidth, height=0.070\linewidth]{figures/qualitative_results/horse-pokemon/source/p_25_000000.png}} & ~~\rotatebox{270}{{\hspace{-3.5em} Source 
  \hspace{-3.0em} } }
  \tabularnewline[-4pt]
\end{tabular}
%%%%%%%%%%%% end first 



\par\end{centering}
\vspace{5pt}
\caption{Visual comparison to prior methods. Visual comparison to prior methods. Visual comparison to prior methods. Visual comparison to prior methods. Visual comparison to prior methods. Visual comparison to prior methods.Visual comparison to prior methods. Visual comparison to prior methods.}
\label{fig:qualitative_comparison_distant2}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}


==> tables/rebuttal_weights_Lall.tex <==
\begin{table}[t]

	\setlength{\tabcolsep}{0.55em}
	\renewcommand{\arraystretch}{0.75}
	\centering
		\begin{tabular}{@{\hskip -0.04in}c@{\hskip 0.04in}|c@{\hskip -0.01in}c@{\hskip 0.02in}|c@{\hskip -0.05in}c@{\hskip -0.06in}}
			\multirow{2}{*}{\footnotesize{} $\mathcal{L}_{all}$ weighting}  & \multicolumn{2}{c|}{\footnotesize{} \hspace{-0.7ex} \textbf{Face$\rightarrow$Anime}} & \multicolumn{2}{c}{\footnotesize{} \hspace{-1.5ex} \textbf{Church$\rightarrow$Shells}} % & \multicolumn{2}{c}{\footnotesize{} \hspace{-1.0ex}\textbf{Horse$\rightarrow$Pokemon}}
            \tabularnewline 
            & \footnotesize{} FID$\downarrow$  & \footnotesize{} LPIPS$\uparrow$  & \footnotesize{} FID$\downarrow$  & \footnotesize{} LPIPS$\uparrow$ % & \footnotesize{} FID$\downarrow$  & \footnotesize{} LPIPS$\uparrow$ 
            \tabularnewline
            
			\hline 	



			{\footnotesize{} ``Earlier''} & \footnotesize{96.8} & \footnotesize{\textbf{0.59}}  & \footnotesize{157.4} & \footnotesize{0.52}  % & \footnotesize{115.0} & \footnotesize{0.52} 
            \tabularnewline

            \footnotesize{} Uniform (ours) & {\footnotesize{97.3}} & \footnotesize{0.57}   & {\footnotesize{140.5}} & \textbf{{\footnotesize{0.53}}} % & \textbf{\footnotesize{84.1}} & \textbf{\footnotesize{0.61}} \tabularnewline
            \tabularnewline
            
            \footnotesize{} ``Later'' & \textbf{\footnotesize{93.2}} & \footnotesize{0.53}  & \textbf{\footnotesize{138.4}} & \footnotesize{0.48}  % & \footnotesize{90.4} & \footnotesize{0.55} 
            

\end{tabular}
%\vspace{0.5ex}
%\caption{Impact of $\mathcal{L}_{all}$ and $\mathcal{L}_{SS}$. Bold denotes best performance.}
\label{table:rebuttal_weigths_Lall} %
\vspace{-2.4ex}
\end{table}
